GitTables: A Large-Scale Corpus of Relational Tables

The success of deep learning has sparked interest in improving relational table tasks, like data preparation and search, with table representation models trained on large table corpora. Existing table corpora primarily contain tables extracted from HTML pages, limiting the capability to represent offline database tables. To train and evaluate high-capacity models for applications beyond the Web, we need resources with tables that resemble relational database tables. Here we introduce GitTables, a corpus of 1M relational tables extracted from GitHub. Our continuing curation aims at growing the corpus to at least 10M tables. Analyses of GitTables show that its structure, content, and topical coverage differ significantly from existing table corpora. We annotate table columns in GitTables with semantic types, hierarchical relations and descriptions from Schema.org and DBpedia. The evaluation of our annotation pipeline on the T2Dv2 benchmark illustrates that our approach provides results on par with human annotations. We present three applications of GitTables, demonstrating its value for learned semantic type detection models, schema completion methods, and benchmarks for table-to-KG matching, data search, and preparation. We make the corpus and code available at https://gittables.github.io.

==> 06_usage.tex <==
\section{Corpus usage}\label{sec:usage}

The rise of machine learning, especially deep learning, is driven by large-scale datasets like \gittables. For \gittables to be useful now, and remain useful in the future, we elaborate on its accessibility, content and usage. 

\subsection{Accessibility}

\gittables is hosted on Zenodo~\cite{zenodo} which ensures versioning and long-term persistence of the corpus. 
The main corpus can be found at \url{https://zenodo.org/record/4943312}. The benchmark dataset for column type detection (e.g. for table-to-KG matching) is hosted at \url{https://zenodo.org/record/5706316}. We will publish the larger corpus with approximately 10M tables as a new dataset on Zenodo. We publish \gittables itself under the Creative Commons Attributions 4.0 International license (CC BY 4.0). All material such as code, documentation, and the used ontologies can be accessed through the website of \gittables: \url{https://gittables.github.io}.


\subsection{Content and structure}
The parsed tables are stored in the Apache Parquet file format, which is widely used for efficiently storing and processing tabular data. Filenames are kept as found on GitHub but in case of filename duplication an identifier is added (e.g.``\_1''). The table metadata (e.g. atomic data types and URL of underlying CSV) and column annotations are stored in the metadata of the file. As each repository license imposes a unique set of rights to the tables that might be important for using the corpus, we add the repository license to the metadata of the files as well.

We publish the corpus in subsets of tables based on the topic used to query them, which enables selection of table subsets depending on a user's needs. The released code\footnote{\url{https://github.com/madelonhulsebos/gittables}} can be used for extracting tables from GitHub for custom query topics depending on the user's interest. As CSV files are of general interest to the data management community, we also publish the raw CSV files.

\subsection{Responsible use}
Despite the many positive applications that our work is intended to have, we recognize that publishing large datasets extracted from the web comes with potential risks. First, it might occur that the CSV files underlying to \gittables still contain sensitive, harmful or otherwise undesired information, despite our effort to suppress this. Making data files accessible at scale may have a negative impact if such undesired content is present.

Second, training models on large datasets extracted from the Web may impose biases~\cite{bender2021dangers}. As illustrated in Section~\ref{sec:bias} data in \gittables mainly reflects English semantics. Models trained on \gittables might therefore be more accurate when applied in English-speaking regions. Despite the scarce presence of semantic types that may impose unwanted biases towards certain subpopluations, we suggest users of \gittables to assess derived artefacts on the presence of such biases before deploying or publishing them.
We ask users to report any observations of biases, harmful content or otherwise undesired data in \gittables by using the contact form on our website.

